Extending OMNeT++ Towards a Platform for the Design of Future In-Vehicle Network Architectures

In-vehicle communication technologies are evolving. While today's cars are equipped with fieldbusses to interconnect the various electronic control units, next generation vehicles have timing and bandwidth requirements that exceed the capacities. In particular Advanced Driver Assistance Systems (ADAS) and automated driving using high bandwidth sensors such as cameras, LIDAR or radar will challenge the in-car network. Automotive Ethernet is the most promising candidate to solve the upcoming challenges. But to design and evaluate new protocols, concepts, and architectures suitable analysis tools are required. Especially in the interim period with architectures using automotive Ethernet and legacy fieldbusses together, careful planning and design is of vital importance. Simulation can provide a good understanding of the expectable network metrics in an early development phase. This paper contributes a workflow as well as the required toolchain to evaluate new real-time Ethernet communication architectures using event based simulation in OMNeT++. We introduce a domain specific language (DSL) - the Abstract Network Description Language (ANDL) - to describe and configure the simulation and present the required simulation models for real-time Ethernet and fieldbus technologies such as CAN and FlexRay. We further introduce new analysis tools for special in-vehicle network use-cases and the interaction of the simulation with third-party applications established in the automotive domain.

==> evaluation.tex <==
\section{Comparative Evaluation}
\label{sec:evaluation}
In the following evaluation, performance results of the event-triggered traffic classes in Ethernet AVB and the rate-constrained class, as well as the scheduled time-triggered traffic are compared for varying cross-traffic loads and frame sizes. We quantify the effect of competing cross-traffic on the prioritized classes.

\subsection{Results}
\subsubsection{Control Traffic}
Control traffic is the most sensitive data transferred within the car. It must comply with the tightest temporal and reliability requirements, since all coordination messages for driving are transmitted therein.
In this scenario, we compare Ethernet AVBs SR class A with the rate-constrained traffic class (for acyclic messages) and the time-triggered traffic (for cyclic messages). The worst-case timing was obtained with messages sent from the HeadUnit to the DME1 ECU (see figure \ref{fig:topology}) in parallel with best-effort cross-traffic from the external data ECU (ED) to DME1. Accordingly, the real-time and best-effort streams share three of their four hops from source to sink. Realistic applications for cross-traffic in this scenario are software updates or diagnosis.

Table \ref{tab:ControlResults} gives an overview of the end-to-end performance for control-traffic in the different real-time traffic classes and cross-traffic bursts at varying frame sizes. As expected, the time-triggered traffic class admits the best results, both for end-to-end latency ($<$\SI{82.03}{\us}) and jitter ($<$\SI{1.17}{\us}) when increasing the frame size of the cross-traffic. Due to the coordinated TDMA approach, the performance is independent of the best-effort traffic. The slight variance in the jitter ($<$\SI{20}{\ns}) is due to the inaccuracy by the clock. The rate-constrained traffic class performs slightly better than time-triggered traffic up to a cross-traffic frame size of approximately \SI{200}{\byte}, but congestion increases latency and jitter for larger frames. Within the scenario, the maximum end-to-end delay for rate-constrained control messages is \SI{258.48}{\us} with cross-traffic of \SI{1518}{\byte}. Ethernet AVB shows the lowest performance for control-traffic with concurrent cross-traffic with a maximum end-to-end latency of \SI{484.27}{\us} (with cross-traffic of max. frame size). %Compared to a configuration without best-effort traffic this is a significant increase of approximately \SI{540}{\percent}.

\begin{table}[]
\centering
\caption{Overview Results for Control Traffic using different real-time Ethernet Technologies and Cross-traffic Frame sizes: Maximum latency and absolute jitter}
\label{tab:ControlResults}  
\begin{tabular}{S[table-format=4] S[table-format=3.2] S[table-format=3.2] S[table-format=1.2] S[table-format=1.2] S[table-format=2.2] S[table-format=2.2]}
\bf{Size}      & \multicolumn{2}{l}{\bf{IEEE 802.1 AVB}}& \multicolumn{2}{l}{\bf{Time-triggered}}& \multicolumn{2}{l}{\bf{Rate-constrained}}\\
\bf{Cr. Tr.}   & \bf{Latency}    & \bf{Jitter}      & \bf{Latency}    & \bf{Jitter}    & \bf{Latency}    & \bf{Jitter}\\
\bf{[\si{\byte}]}    & \bf{[\si{\us}]}& \bf{[\si{\us}]} & \bf{[\si{\us}]}&\bf{[\si{\us}]}& \bf{[\si{\us}]}&\bf{[\si{\us}]} \\\hline\hline
0              & 75.69           & 7.23             & 82.02           & 1.17           & 42.26           & 19.12\\
100            & 142.97          & 10.58            & 82.03           & 1.16           & 70.95           & 47.81\\
800            & 344.64          & 69.60            & 82.02           & 1.15           & 162.57          & 139.43\\
1518           & 484.27          & 112.82           & 82.02           & 1.16           & 258.48          & 235.34\\
\end{tabular}
%\vspace{-5mm}
\end{table}

Figure \ref{fig:ed_dme1_max} visualizes the dependency between the cross-traffic frame size and the maximum end-to-end latency of the real-time control traffic for the unscheduled traffic classes (AVB and rate-constrained). The time-triggered end-to-end latency remains unaffected by the cross-traffic. In the average case, rate-constrained traffic exceptionally suffers from larger packets. This is due to the increased probability of two packets residing at the same time in the output queue of outgoing line cards. For Ethernet AVB the absolute latency is even larger, but due to the dominance of the delay of the credit-based shaper we see a more linear increase for larger packets.

\begin{figure}[!b]
\centering
\vspace{-0.5mm}
\includegraphics[width=1\columnwidth]{../origin/ed_dme1_avg_max.pdf}
%\vspace{-6mm}
\caption{Maximum end-to-end latency of real-time control traffic in relation to the maximum frame size of concurrent best-effort cross-traffic}
\label{fig:ed_dme1_max}
\end{figure}


\subsubsection{Camera Streams of Driver Assistance}
The driver assistance camera stream composed by the DA\_CAM ECU consists of a stitched surround image stream with \SI{25}{\mega\bit\per\second}. The stream is forwarded to the Display1-ECU. The external data ECU (ED) sends concurrent cross-traffic representing e.g. media streaming or off-board navigation data. In this case only one hop suffers from concurrency of real-time and cross-traffic, thus the influences on the end-to-end latency and jitter are smaller than for the control traffic. As the media streams are not synchronized and thus not suitable for time-triggered traffic we compare AVBs class A with rate-constrained traffic.

The Ethernet AVB traffic class performs much better in this scenario compared to the control traffic (see table \ref{tab:DAResults}). For cross-traffic with \SI{1518}{\byte}, the maximum end-to-end latency is bounded at \SI{211.70}{\us} compared to \SI{311.37}{\us} for the rate-constrained traffic. In the average case both, traffic using AVBs credit based shaper and rate-constrained traffic performs equally well. For Ethernet AVB, the average end-to-end latency increases with larger frames by approximately \SI{3}{\percent} from \SI{108.70}{\us} to \SI{112.05}{\us}. For rate-constrained traffic the increase is approximately \SI{6}{\percent} from \SI{100.34}{\us} to \SI{106.38}{\us}. This shows that the probability of cross-traffic delaying frames of the camera stream is low. Figure \ref{fig:ed_display1_max} shows a comparison of the maximum and average end-to-end latency of both classes.

\begin{table}[]
\centering
\caption{Overview Results for Driver Assistance Camera Traffic using different real-time Ethernet Technologies and Cross-traffic Frame Sizes: Maximum latency and absolute jitter}
\label{tab:DAResults}  
\begin{tabular}{S[table-format=4] S[table-format=3.2] S[table-format=2.2] S[table-format=3.2] S[table-format=3.2]}
\bf{Frame Size}     & \multicolumn{2}{l}{\bf{IEEE 802.1 AVB}}& \multicolumn{2}{l}{\bf{Rate-constrained}}\\
\bf{Cross-traffic} & \bf{Latency}    & \bf{Jitter}      & \bf{Latency}    & \bf{Jitter}\\
\bf{[\si{\byte}]}        & \bf{[\si{\us}]}& \bf{[\si{\us}]} & \bf{[\si{\us}]}&\bf{[\si{\us}]} \\\hline\hline
0                  & 108.71         &   17.51           & 211.34          & 111.43         \\
100                & 140.27         &   20.75           & 214.75	          & 114.83         \\
800                & 167.77         &   38.87           & 255.98          & 156.06         \\
1518               & 211.70         &   59.30           & 311.37          & 211.45         \\
\end{tabular}
%\vspace{-5mm}
\end{table}


\begin{figure}[!b]
\centering
%\vspace{-4mm}
\includegraphics[width=1\columnwidth]{../origin/ed_display1_avg_max.pdf}
%\vspace{-6mm}
\caption{Maximum end-to-end latency of real-time driver assistance camera traffic in relation to the maximum frame size of concurrent cross-traffic}
\label{fig:ed_display1_max}
\end{figure}

\subsubsection{Multimedia and Entertainment}
For the multimedia domain we exemplarily show the traffic of the audio streams between the multimedia streaming ECU and the amplifier. Again, the asynchronous characteristics of the traffic make the usage of time-triggered messages inadequate.

Due to the lower priorities chosen for the streams of the entertainment domain, the end-to-end latency and jitter is higher than in the other scenarios. For Ethernet AVB the end-to-end latency is between \SI{497.67}{\us} and \SI{561.51}{\us} depending on the cross-traffic configuration. For rate-constrained traffic with strict priorities the end-to-end latency ranges from \SI{582.58}{\us} to \SI{713.24}. Both, latency and jitter are higher for rate-constrained traffic than for Ethernet AVB. Table \ref{tab:MMResults} shows a comparison of the results for selected frame sizes of cross-traffic.




\subsubsection{Cross-traffic Performance}
In all scenarios the best-effort cross-traffic heavily suffers from the concurrent real-time messages in the network. The highest latencies were simulated on the path between the ED and DME1 ECUs. The maximum latency of individual background cross-traffic frames is at minimum \SI{146.55}{\us} for minimum size frames and goes up to \SI{755.23}{\us} for frames with \SI{1500}{\byte} of payload. For the whole burst the latency decreases with larger packets, starting with \SI{18.85}{\ms} for the smallest packets going down to \SI{11.26}{\ms} for bursts with the largest frames. This decrease is due to the lower overhead when using larger frames. Compared to the latencies obtained in cellular and wide area networks, the simulated cross-traffic latencies are still low. Though it is well suitable for the projected applications in the domains of diagnosis, firmware updates or functions deployed off-board.



\subsubsection{Buffer Sizes}
\label{sec:buffersizes}
Another challenge for in-car networks with cross-traffic bursts is the required buffer size in the forwarding switches. When only smallest frames are used for cross-traffic in this scenario, the queues in the switches are required to host at maximum \SI{1764}{frames} or \SI{110.25}{\kilo\byte}. With only maximum sized frames for cross-traffic the largest fill level of the buffers in the network is \SI{55}{frames} or \SI{81.53}{\kilo\byte}. For real-time frames (that use dedicated queues for each stream) the buffers remain small. Due to the shaping, the maximum sizes for the event-triggered traffic classes remains below \SI{3}{frames}. For time-triggered messages the maximum buffer size in the switches is by definition between \SI{0}{frames} and \SI{1}{frame}.


\begin{table}[]
\centering
\caption{Overview Results for Multimedia and Entertainment using different real-time Ethernet Technologies and Cross-traffic Frame Sizes: Maximum latency and absolute jitter}
\label{tab:MMResults}  
\begin{tabular}{S[table-format=4] S[table-format=3.2] S[table-format=3.2] S[table-format=3.2] S[table-format=3.2]}
\bf{Frame Size}     & \multicolumn{2}{l}{\bf{IEEE 802.1 AVB}}& \multicolumn{2}{l}{\bf{Rate-constrained}}\\
\bf{Cross-traffic} & \bf{Latency}    & \bf{Jitter}      & \bf{Latency}    & \bf{Jitter}\\
\bf{[\si{\byte}]}        & \bf{[\si{\us}]}& \bf{[\si{\us}]} & \bf{[\si{\us}]}&\bf{[\si{\us}]} \\\hline\hline
0                  & 497.67         &   30.23           & 582.58          & 117.20         \\
100                & 518.66         &   36.39           & 592.49	          & 127.11         \\
800                & 539.12         &   90.42           & 646.66          & 181.28         \\
1518               & 561.51         &   105.60          & 713.24          & 252.13         \\
\end{tabular}
%\vspace{0.6mm}
\vspace{-1mm}
\end{table}

\subsection{Discussion}
The simulation results show a diverse behavior of the different technologies when stressed with cross-traffic. For the control traffic the best results are undoubtedly obtained with time-triggered traffic. It was shown that time-triggered traffic proves its promise of determinism and independence of concurrent traffic streams. Also, it was the only traffic class able to comply with the highest end-to-end latency requirements of below \SI{100}{\us} that are under discussion in the automotive industry \cite{tccl-aetsi-15}. There is a controversy whether such low-latency requirements will be really required in the near future. For applications with less rigid timing requirements, Ethernet AVB or its counterpart rate-constrained traffic that use strict priorities along with traffic shaping, still perform sufficiently well with latency bounds below \SI{500}{\us}. For control-traffic the rate-constrained message class slightly performs better than Ethernet AVB due to the absence of credit-based shaping. While rate-constrained traffic with the highest priority only has to wait until the line card is idle, Ethernet AVBs credit based shaper adds a delay in situations where a frame has to wait for enough credit. As the additional delays for real-time messages due to cross-traffic occur for each hop, the penalty of best-effort background traffic increases with the length of the path from sender to receiver.

When utilized for multimedia traffic, Ethernet AVB can provide best results. Especially for the driver assistance camera that is transferred in the highest service class A, the latency influence of cross-traffic is low. Also, the rate-constrained traffic is a possible candidate for driver assistance applications, although adding a delay compared to Ethernet AVB. An even bigger difference between rate-constrained and Ethernet AVB traffic was obtained for the streams of the entertainment domain. With cross-traffic the end-to-end latency of AVB is almost one third lower than for the same streams using rate-constrained traffic. One reason for the performance advantage of Ethernet AVB in the camera and entertainment domain is the concurrent time-triggered traffic in the rate-constrained scenario. In relation to the requirements for audio and video streams both technologies offer sufficient performance.

